Protecting Quantum Procrastinators with Signature Lifting: A Case Study in Cryptocurrencies

Current solutions to quantum vulnerabilities of widely used cryptographic schemes involve migrating users to post-quantum schemes before quantum attacks become feasible. This work deals with protecting quantum procrastinators: users that failed to migrate to post-quantum cryptography in time. To address this problem in the context of digital signatures, we introduce a technique called signature lifting, that allows us to lift a deployed pre-quantum signature scheme satisfying a certain property to a post-quantum signature scheme that uses the same keys. Informally, the said property is that a post-quantum one-way function is used "somewhere along the way" to derive the public-key from the secret-key. Our constructions of signature lifting relies heavily on the post-quantum digital signature scheme Picnic (Chase et al., CCS'17). Our main case-study is cryptocurrencies, where this property holds in two scenarios: when the public-key is generated via a key-derivation function or when the public-key hash is posted instead of the public-key itself. We propose a modification, based on signature lifting, that can be applied in many cryptocurrencies for securely spending pre-quantum coins in presence of quantum adversaries. Our construction improves upon existing constructions in two major ways: it is not limited to pre-quantum coins whose ECDSA public-key has been kept secret (and in particular, it handles all coins that are stored in addresses generated by HD wallets), and it does not require access to post-quantum coins or using side payments to pay for posting the transaction.

==> title_authors_toc.tex <==
% \ifnum\masterthesis=0 
%     \title{Template for Papers    %\ifdraft{\\(working draft)}
%     }
% \fi

% \ifnum\anonymous=0
%     \ifnum\preprint=1
%         \author[1]{XXX}
%         \author[1]{Or Sattath}
%         \affil[1]{Computer Science Department, Ben-Gurion University of the Negev}
%     \fi
%     \ifnum\cryptology=1
%         \author{XXX}
%         \affil{Department of Computer Science, Ben Gurion University of the Negev, Beersheba, Israel\\
%         XXX@post.bgu.ac.il}
%         \author{Or Sattath}
%         \affil{Department of Computer Science, Ben Gurion University of the Negev, Beersheba, Israel\\
%         sattath@bgu.ac.il}
%     \fi
%     \ifnum\sigconf=1
%         \author[1]{XXX}
%         \author[1]{Or Sattath}
%         \affil[1]{Computer Science Department, Ben-Gurion University of the Negev}
%     \fi
%     \ifnum\llncs=1
%         %\titlerunning{Abbreviated paper title}
%         % If the paper title is too long for the running head, you can set
%         % an abbreviated paper title here
%         %
%         \author{Or Sattath\inst{1}\orcidID{0000-0001-7567-3822} \and
%         Second Author\inst{2,3}\orcidID{1111-2222-3333-4444} \and
%         Third Author\inst{3}\orcidID{2222--3333-4444-5555}}
%         %
%         \authorrunning{O. Sattath}
%         % First names are abbreviated in the running head.
%         % If there are more than two authors, 'et al.' is used.
%         %
%         \institute{Department of Computer Science, Ben Gurion University of the Negev, Beersheba, Israel 
%         \email{sattath@bgu.ac.il}\\
%         \url{http://www.springer.com/gp/computer-science/lncs} \and
%         ABC Institute, Rupert-Karls-University Heidelberg, Heidelberg, Germany\\
%         \email{\{abc,lncs\}@uni-heidelberg.de}}
%     \fi
%     \ifnum\quantumjournal=1
%         \author[1]{Andrea Coladangelo}
%         \affil[1]{Computing and Mathematical Sciences,	
%         Caltech}
%         \author[2]{Or Sattath}
%         \orcid{0000-0001-7567-3822}
%         \email{sattath@bgu.ac.il}

%         \affil[2]{Computer Science Department, Ben-Gurion University of the Negev}
        
%     \fi
% \else
%     \ifnum\lipics=0
%         \author{}
%     \fi
% \fi



% \ifthenelse{\equal{\masterthesis}{0} \AND \equal{\sigconf}{0}}{
%     \maketitle
% } 
% {}        
% \ifnum\masterthesis=1
%     \include{masterthesis_header}
% \else 
%     \ifnum\sigconf=0
%         \begin{abstract}
%     \fi
% \fi
% \ifnum\sigconf=0
%     \ifnum\masterthesis=0
% %IN ARXIV SUBMISSIONS, REMEMBER TO INDENT NEW PARAGRAPHS SINCE NEWLINES ARE IGNORED. 

%    Standard abstract goes here. Remember that when submitting the abstract to the arXiv, every new paragraph which is submitted must be indented (start with a few white spaces). New lines (carriage returns) are automatically truncated.
%     \fi
% \fi 
% \ifnum\masterthesis=0
%     \ifnum\sigconf=0
%         \end{abstract}
%     \fi
% \fi

% \ifnum\sigconf=1
%     \begin{abstract}
%         Abstract of SigConf goes here.
%     \end{abstract}
%     \keywords{}
%     \maketitle
% \fi

% \ifnum\toc=1
%     \ifnum\llncs=1
%         \setcounter{secnumdepth}{3}
%         \setcounter{tocdepth}{3}
%     \fi
%     \tableofcontents 
% \fi
